Network Sparsification for Steiner Problems on Planar and Bounded-Genus Graphs

We propose polynomial-time algorithms that sparsify planar and bounded-genus graphs while preserving optimal or near-optimal solutions to Steiner problems. Our main contribution is a polynomial-time algorithm that, given an unweighted graph $G$ embedded on a surface of genus $g$ and a designated face $f$ bounded by a simple cycle of length $k$, uncovers a set $F \subseteq E(G)$ of size polynomial in $g$ and $k$ that contains an optimal Steiner tree for any set of terminals that is a subset of the vertices of $f$. We apply this general theorem to prove that: * given an unweighted graph $G$ embedded on a surface of genus $g$ and a terminal set $S \subseteq V(G)$, one can in polynomial time find a set $F \subseteq E(G)$ that contains an optimal Steiner tree $T$ for $S$ and that has size polynomial in $g$ and $|E(T)|$; * an analogous result holds for an optimal Steiner forest for a set $S$ of terminal pairs; * given an unweighted planar graph $G$ and a terminal set $S \subseteq V(G)$, one can in polynomial time find a set $F \subseteq E(G)$ that contains an optimal (edge) multiway cut $C$ separating $S$ and that has size polynomial in $|C|$. In the language of parameterized complexity, these results imply the first polynomial kernels for Steiner Tree and Steiner Forest on planar and bounded-genus graphs (parameterized by the size of the tree and forest, respectively) and for (Edge) Multiway Cut on planar graphs (parameterized by the size of the cutset). Additionally, we obtain a weighted variant of our main contribution.

==> weighted-old-single-pair.tex <==

\subsection{Single-pair case}\label{ss:wei:paths}

We start with 
The goal of this section is to prove the following single-pair variant of
Theorem~\ref{thm:weighted}:

\begin{theorem}\label{thm:wei:paths}
Let $\eps > 0$ be a fixed accuracy parameter,
and let $B$ be an edge-weighted brick.
Then one can find in $\Oh(\eps^{-2} |B| \log |B|)$ time a graph
$H \subseteq B$ such that
\begin{enumerate}
\item $\prm B \subseteq H$,
  \item $\wei{H} = \Oh(\eps^{-5} \wei{\prm B})$, and
  \item for any pair of vertices $s,t \in V(\prm B)$
there exists a path connecting $s$ and $t$ in $H$
of weight at most $(1+\eps)\dist_B(s,t)$.
\end{enumerate}
\end{theorem}

We prove Theorem~\ref{thm:wei:paths} in two steps. First, we observe
that it suffices to look only at special types of bricks, called \emph{strips},
introduced by Klein~\cite{klein:stoc06}.
Intuitively, each strip looks like a long eye-shaped brick, with its perimeter being a union
of two (almost) shortest paths.
Second, we show that in a strip it suffices to take as $H$ only a small number
of shortest paths, somewhat resembling vertical `columns' in an eye-shaped strip.

\subsubsection{Strips}

Let $\eps > 0$ be fixed and, without loss of generality, assume $\eps < \frac{1}{2}$.
We need the following notions from~\cite{klein:stoc06,klein:planar-st-eptas} (phrased in our terminology).
\begin{definition}[$\eps$-short path, \cite{klein:planar-st-eptas}]
A path $P$ in a graph $G$ is \emph{$\eps$-short in $G$}
if for every two vertices $x,y \in V(P)$ 
we have $\dist_P(x,y) \leq (1+\eps)\dist_G(x,y)$.
\end{definition}

\begin{definition}[strip, \cite{klein:stoc06,klein:planar-st-eptas}]
A brick $B$ is called a \emph{strip} if $\prm B$ can be decomposed into two
nonempty paths $\north$ and $\south$ such that in $B$:
(a) $\south$ is a shortest path between its endpoints,
and (b) every proper subpath of $\north$ is an $\eps$-short path.
\end{definition}

The paths $\north$ and $\south$ are called \emph{north} and \emph{south} boundary
of the strip $B$. If one travels $\prm B$ in the counter-clockwise direction,
the first vertex of $\south$ is called the \emph{leftmost} vertex of $\south$
and the last vertex is the \emph{rightmost} vertex of $\south$.
Note that both these vertices are also endpoints of $\north$.

\begin{lemma}[\cite{klein:stoc06,klein:planar-st-eptas}]\label{lem:strips}
There exists an algorithm that, given a brick $B$,
in $\Oh(|B| \log |B|)$ time finds a $(2\eps^{-1}+3)$-short
brick partition $\Bb=\{B_1,\ldots,B_p\}$ of $B$,
such that $B_i$ is a strip for every $1 \leq i \leq p$.
Moreover, within the same running time,
the algorithm can also provide the partition of $\prm B_i$ into paths $\north$ and $\south$
for every $1 \leq i \leq p$.
\end{lemma}

Using Lemma~\ref{lem:strips}, we can show that it suffices to prove the following theorem:
\begin{theorem}\label{thm:wei:strips}
Let $\eps > 0$ be a fixed accuracy parameter,
and let $B$ be an edge-weighted strip with given north and south boundary.
Then one can find in $\Oh(\eps^{-2} |B| \log |B|)$ time a graph
$H \subseteq B$ such that
\begin{enumerate}
\item $\prm B \subseteq H$,
  \item $\wei{H} = \Oh(\eps^{-4} \wei{\prm B})$, and
  \item for any pair of vertices $s,t \in V(\prm B)$
there exists a path connecting $s$ and $t$ in $H$ of length at most $(1+\eps)\dist_B(s,t)$.
\end{enumerate}
\end{theorem}
\noindent
Indeed, using Lemma~\ref{lem:strips} and Theorem~\ref{thm:wei:strips}, we can prove Theorem~\ref{thm:wei:paths} as follows:

\begin{proof}[Proof of Theorem~\ref{thm:wei:paths}]
Apply Lemma~\ref{lem:strips} to the input brick $B$, and let $\Bb=\{B_1,\ldots,B_p\}$ be the resulting brick partition, where each $B_{i}$ is a strip. Apply the algorithm of Theorem~\ref{thm:wei:strips} to each strip $B_{i}$, and let $H_{i}$ denote the resulting subgraph of $B_{i}$.
We claim that $H := \bigcup_{i=1}^p H_i$ satisfies all requirements of Theorem~\ref{thm:wei:paths}.
Since $\Bb$ is a brick partition of $B$, $\prm B \subseteq H$. Moreover, $H$ can be computed in total $\Oh(\eps^{-2} |B| \log |B|)$ time due to the time
bounds of Lemma~\ref{lem:strips} and Theorem~\ref{thm:wei:strips}, and the fact that each edge of $B$ belongs to at most two
strips $B_i$ (since $\Bb$ is a brick partition of $B$).

 Consider any pair $s,t \in V(\prm B)$ and let $Q$ be a shortest path between $s$ and $t$
in the brick $B$. Let $Q'$ be any maximal subpath of $Q$ that consists only
of edges strictly enclosed by $\prm B_i$ for some $1 \leq i \leq p$, and let
$s',t'$ be the endpoints of $Q'$. By the properties of $H_i$, there exists
a path $P' \subseteq H_i$ of length at most $(1+\eps)\wei{P'}$ with endpoints $s'$ and $t'$.
Moreover, observe that all such subpaths $Q'$ of $Q$ are pairwise edge-disjoint.
Hence, we may replace each such subpath $Q'$ with the path $P'$ defined as above,
obtaining a walk $P$ connecting $s$ and $t$ of length at most $(1+\eps)\wei{Q}$.
As $\prm B_{i} \subseteq H$ for each $1 \leq i \leq p$ and each constructed path $P'$ is contained in some graph $H_i$, we have $P \subseteq H$.
Finally, observe that since $\Bb$ is $(2\eps^{-1}+3)$-short,
$$\wei{\bigcup_{i=1}^p H_i} \leq \sum_{i=1}^p \wei{H_i} \leq \sum_{i=1}^p \Oh(\eps^{-4} \wei{\prm B_i}) = \Oh(\eps^{-5} \wei{\prm B}).$$
The theorem follows.
\end{proof}

\subsubsection{Columns}
In the remainder of this section, we aim to prove Theorem~\ref{thm:wei:strips}. Let $B$ denote the strip, and let $\north$ and $\south$ denote the partition of $\prm B$ as per definition.
Let $\Bleft$ and $\Bright$ be the leftmost and rightmost vertex of $\south$, respectively.
Recall that $\Bleft$ and $\Bright$ are endpoints of both $\north$ and $\south$.

We now identify \emph{columns} in the strip $B$ in a similar, but slightly different, way as in~\cite{klein:stoc06,klein:planar-st-eptas}.
Define $x_0 := \Bleft$ and traverse $\north$ starting from the endpoint $x_0$.
For $i=1,2,\ldots$, find the first vertex $x_i$ on $\north$ such that
$\dist_\north(x_{i-1},x_i) > \eps \dist_B(x_{i-1},\south)$.
Define column $C_i$ to be some arbitrarily chosen shortest path between $x_i$ and $\south$ in $B$ and let $y_i$ be the other endpoint of $C_i$.
Let $x_q$ be the last vertex defined in this way.
Observe that $x_q = \Bright$, as otherwise $\dist_\north(x_q,\Bright) \geq \dist_B(x_q,\Bright) \geq \dist_B(x_q,\south)$ and, since $\eps < \frac{1}{2}$,
the vertex $\Bright$ is a feasible candidate for $x_{q+1}$.

\begin{figure}[htbp!]
        \centering
                \def\svgwidth{0.9\textwidth}
                \input{figures/strip.pdf_tex}
\caption{Construction of columns in a strip.}\label{fig:strip}
\end{figure}

Similarly as in~\cite{klein:stoc06}, we can bound the total length of columns and find them efficiently.

\begin{lemma}\label{lem:wei:colbound}
The sum of the length of the columns is bounded by $\eps^{-1} \wei{\north} \leq \eps^{-1} \wei{\prm B}$.
\end{lemma}
\begin{proof}
As $x_q = \Bright$, we have $\wei{C_q} = 0$. For the other columns, by construction and the definition of $\north$:
$$\sum_{i=0}^{q-1} \wei{C_i} = \sum_{i=0}^{q-1} \dist_B(x_i,\south) < \eps^{-1} \dist_\north(x_i,x_{i+1}) = \eps^{-1} \wei{\north}.$$
\end{proof}

\begin{lemma}\label{lem:wei:colfind}
One can identify the vertices $x_0,x_1,\ldots,x_q$, distances $\dist_B(x_i,\south)$ for $0 \leq i \leq q$,
vertices $y_0,y_1,\ldots,y_q$, and the edge set $\bigcup_{i=0}^q C_i$ for some choice of columns $C_i$, in $\Oh(|B|)$ time.
\end{lemma}
\begin{proof}
Create a new super-terminal $t$ in the outer face of $B$, connect it with zero-length edges to all vertices of $V(\south)$,
%and perform the single-source shortest path algorithm from $t$ in the resulting planar graph, obtaining 
and find a shortest-path tree $T$ rooted at $t$ in the resulting planar graph. This takes linear time~\cite{planar-sp}.
Using the tree, one can identify for each $v \in V(B)$ both the distance $\dist_B(v,\south)$ and some closest vertex $y(v) \in V(\south)$.
With this information, it is straightforward to identify the vertices $x_i$, $y_i$ and values $\dist_B(x_i,\south)$, where the column $C_i$
is taken as the subpath in $T$ between the vertex $x_i$ and its ancestor $y_i := y(x_i) \in V(\south)$ on the path to the root $t$.
Moreover, by traversing the tree $T$ in a bottom-up fashion, one can in linear time mark all the edges of $\bigcup_{i=0}^q C_i$
for this particular choice of columns $C_i$.
\end{proof}
We remark that the columns $C_i$ computed by the algorithm of Lemma~\ref{lem:wei:colfind} are non-crossing in the following sense:
whenever $C_i$ and $C_j$ meet at some point, they continue together to a common endpoint $y_i=y_j$.
However, we will not use this property in the sequel.

\subsubsection{Pegs}

The idea of the construction of the subgraph $H$ of $B$ is as follows: either the shortest path between the given terminals $s$ and $t$
goes along one column $C_i$, or it is more-or-less horizontal. In the first case, we hope to handle it by adding to $H$ a few shortest paths that are close to $C_i$.
In the second case, some column $C_{i}$ should have negligible length compared to the length of such a path, and thus the columns $C_i$ together
with $\prm B$ should suffice to handle such a pair $(s,t)$.

We now establish how to handle terminal pairs $(s,t)$ where the shortest path between $s$ and $t$ in $B$ is in some sense close to some column $C_i$.
Fix one index $i$, $0 \leq i \leq q$, and define $z_{i,0} := y_i$.
Traverse $\south$ to the right (in the direction of $\Bright$), starting from $z_{i,0}$.
For each $j = 1,2,\ldots$ define $z_{i,j}$ to be the first vertex satisfying $\dist_\south(z_{i,j-1},z_{i,j}) > \eps \wei{C_i}$.
Symmetrically, traverse $\south$ to the left (in the direction of $\Bleft$), starting from $z_{i,0}$. For each $j=1,2,\ldots$, define $z_{i,-j}$ to be the first vertex satisfying $\dist_\south(z_{i,-(j-1)},z_{i,-j}) > \eps \wei{C_i}$.
The vertices $z_{i,j}$ are called \emph{pegs} for the column $C_i$.
Define $r_\rightarrow(i)$ to be the last index $j$ for which $\dist_\south(y_i,z_{i,j}) \leq \eps^{-1} \wei{C_i}$,
and $r_\leftarrow(i)$ to be the last index $j$ for which $\dist_\south(y_i,z_{i,-j}) \leq \eps^{-1} \wei{C_i}$.
Observe that 
\begin{equation}\label{eq:wei:paths:r-bound}
r_\rightarrow(i),r_\leftarrow(i) \leq \eps^{-2}.
\end{equation}

For every $-r_\leftarrow(i) \leq j \leq r_\rightarrow(i)$ define the \emph{cord} $P_{i,j}$ to be some arbitrarily chosen
shortest path in $B$ between $x_i$ and $z_{i,j}$. In what follows we show that
\begin{equation}\label{eq:wei:paths:H}
H := \prm B \cup \bigcup_{i=0}^q \bigcup_{j=-r_\leftarrow(i)}^{r_\rightarrow(i)} P_{i,j}
\end{equation}
satisfies all the desired conditions for the subgraph $H$ and, moreover, it can be computed efficiently for some choice of cords $P_{i,j}$.

\begin{figure}[htbp!]
        \centering
                \def\svgwidth{0.9\textwidth}
                \input{figures/column.pdf_tex}
\caption{Construction of pegs $z_{i,j}$ and cords $P_{i,j}$ (in grey) for one column $C_i$.}\label{fig:column}
\end{figure}

\subsubsection{Correctness}

We first show that the graph $H$ defined in~\eqref{eq:wei:paths:H} preserves approximate shortest paths between pairs of vertices on $\prm B$.

\begin{lemma}\label{lem:wei:paths:correct}
For any $s,t \in V(\prm B)$, it holds that $\dist_H(s,t) \leq (1+12\eps) \dist_B(s,t)$.
\end{lemma}
\begin{proof}
If both $s$ and $t$ belong to $V(\south)$ or both $s$ and $t$ belong to $V(\north)$,
then the claim is straightforward, as $\prm B \subseteq H$, $\south$ is a shortest path in $B$, and any proper subpath of $\north$ is $\eps$-short in $B$.
Hence, we may restrict ourselves to the case $s \in V(\north)$, $t \in V(\south)$.

Let $0 \leq i < q$ be an index such that $s$ lies on the subpath of $\north$ between $x_i$ and $x_{i+1}$ (possibly $s = x_i$, but $s \neq x_{i+1}$).
By the choice of $x_{i+1}$,
\begin{equation}\label{eq:wei:paths:correct:1}
\dist_B(s,x_{i}) \leq  \dist_\north(s,x_i) \leq \eps\, \wei{C_i} = \eps\, \dist_B(x_i,\south).
\end{equation}
As $t \in V(\south)$, it follows from~\eqref{eq:wei:paths:correct:1} that
\begin{equation}\label{eq:wei:paths:correct:2}
\dist_B(s,t) \geq \dist_B(s,\south) \geq \dist_B(x_i,\south) - \dist_B(s,x_i) \geq (1-\eps)\wei{C_i}.
\end{equation}

Without loss of generality, assume that $t$ lies on $\south$ between $y_i = z_{i,0}$ and $\Bright$ (possibly $t=y_i$); the second case will be symmetrical.
We now consider two cases, depending on $\dist_\south(y_i,t)$.
If $\dist_\south(y_i,t) \leq \eps^{-1} \wei{C_i}$, then let $j$ be the last index such that $z_{i,j}$ lies on the path $\south$
between $y_i$ and $t$ (possibly $t = z_{i,j}$). By the definition of the sequence $z_{i,j}$, we have $\dist_\south(z_{i,j},t) \leq \eps \wei{C_i}$.
By the definition of $r_\rightarrow(i)$, we have $j \leq r_\rightarrow(i)$. Note that the cord $P_{i,j}$ is contained in $H$.
Consider the following path between $s$ and $t$ in $H$: we first go along $\north$ to $x_i$, then traverse $P_{i,j}$ to $z_{i,j}$, and then continue
along $\south$ to $t$. We obtain:
\begin{equation}\label{eq:wei:paths:correct:3}
\dist_H(s,t) \leq \dist_\north(s,x_i) + \wei{P_{i,j}} + \dist_\south(z_{i,j},t) \leq 2\eps \wei{C_i} + \dist_B(x_i,z_{i,j}).
\end{equation}
However, 
\begin{equation}\label{eq:wei:paths:correct:4}
\dist_B(x_i,z_{i,j}) \leq \dist_B(x_i,s) + \dist_B(s,t) + \dist_B(t,z_{i,j}) \leq 2\eps\wei{C_i} + \dist_B(s,t).
\end{equation}
By combining \eqref{eq:wei:paths:correct:2}, \eqref{eq:wei:paths:correct:3} and \eqref{eq:wei:paths:correct:4} we obtain
$$\dist_H(s,t) \leq 4\eps\wei{C_i} + \dist_B(s,t) \leq \left(1+\frac{4\eps}{1-\eps}\right) \dist_B(s,t) < (1+8\eps)\dist_B(s,t),$$
where the last inequality follows from the assumption that $\eps < \frac{1}{2}$.

In the remaining case, $\dist_\south(y_i,t) > \eps^{-1} \wei{C_i}$ and, consequently,
\begin{eqnarray}\label{eq:wei:paths:correct:5}
\dist_B(s,t) & \geq & \dist_B(y_i,t) - \dist_B(x_i,y_i) - \dist_B(s,x_i) \nonumber \\
& \geq & \dist_\south(y_i,t) - (1+\eps)\wei{C_i} \nonumber \\
& > & (\eps^{-1} - 1 - \eps) \wei{C_i}.
\end{eqnarray}
Moreover,
\begin{eqnarray}\label{eq:wei:paths:correct:6}
\dist_{\south}(y_{i},t) & = & \dist_{B}(y_{i},t) \nonumber\\
& \leq & \dist_{B}(s,t) + \dist_{B}(s,x_{i}) + \dist_{B}(x_{i},y_{i})  \nonumber\\
& \leq & \dist_{B}(s,t) + (1+\eps)\wei{C_{i}}.
\end{eqnarray}
Consider the following path connecting $s$ and $t$ in $H$: we first traverse $\north$ from $s$ to $x_i$, then we go along the cord $P_{i,0}$, and then we traverse $\south$ from $y_i$ to $t$.
Since this path exists in $H$ and by~\eqref{eq:wei:paths:correct:5} and ~\eqref{eq:wei:paths:correct:6}, we obtain that:
\begin{align*}
\dist_H(s,t) &\leq \dist_\north(s,x_i) + \wei{P_{i,0}} + \dist_\south(y_i,t) \\
    &\leq (1+\eps)\wei{C_i} + \dist_B(s,t) + (1+\eps)\wei{C_i} \\
    &\leq \dist_B(s,t) + (2+2\eps)\wei{C_i} \\
    &< \dist_B(s,t) + \frac{2+2\eps}{\eps^{-1}-1-\eps} \dist_B(s,t) \\
    &< (1+12\eps)\dist_B(s,t),
\end{align*}
where the last inequality follows from the assumption that $\eps < \frac{1}{2}$. The lemma follows.
\end{proof}

\subsubsection{Bound on the length of $H$}

We now bound the total length of the graph $H$.
\begin{lemma}\label{lem:wei:paths:length}
The graph $H$ defined in~\eqref{eq:wei:paths:H} has total length $\Oh(\eps^{-4} \wei{\prm B})$.
\end{lemma}
\begin{proof}
Observe that for any vertex $x_i$ and any peg $z_{i,j}$ with $-r_\leftarrow(i) \leq j \leq r_\rightarrow(i)$
we have
\begin{equation}\label{eq:wei:paths:length1}
\wei{P_{i,j}} = \dist_B(x_i,z_{i,j}) \leq \dist_B(x_i,y_i) + \dist_B(y_i,z_{i,j}) \leq (1+\eps^{-1}) \wei{C_i}.
\end{equation}
Hence,
\begin{align*}
\wei{H} &\leq \wei{\prm B} + \sum_{i=0}^q \sum_{j=-r_\leftarrow(i)}^{r_\rightarrow(i)} \wei{P_{i,j}} & \textrm{by definition of }H\\
        &\leq \wei{\prm B} + \sum_{i=0}^q \left(1+r_\leftarrow(i)+r_\rightarrow(i)\right)(1+\eps^{-1}) \wei{C_i} & \textrm{by~\eqref{eq:wei:paths:length1}}\\
        &\leq \wei{\prm B} + \sum_{i=0}^q (1+\eps^{-1})(1+2\eps^{-2}) \wei{C_i}& \textrm{by~\eqref{eq:wei:paths:r-bound}}\\
        &\leq \wei{\prm B} + (1+\eps^{-1})(1+2\eps^{-2})\eps^{-1} \wei{\prm B}& \textrm{by Lemma~\ref{lem:wei:colbound}}\\
        &= \Oh(\eps^{-4} \wei{\prm B}) &\textrm{as }\eps < \frac{1}{2}.
\end{align*}
\end{proof}

\subsubsection{Efficient computation of $H$}

To finish the proof of Theorem~\ref{thm:wei:strips}, we need to show how to compute the graph $H$ in $\Oh(\eps^{-2} |B| \log |B|)$ time.
Observe that a naive implementation uses $\Oh(|B|\log |B|)$ time for each vertex $x_i$, giving a $\Oh(|B|^2\log |B|)$ time bound.
This is because we do not control $q$, the number of vertices $x_i$.
We improve the running time using the multiple-source shortest path algorithm of Klein~\cite{klein:mssp}.

\begin{lemma}\label{lem:wei:paths:time}
The graph $H$ defined in~\eqref{eq:wei:paths:H} can be computed in
  $\Oh(\eps^{-2}|B|\log |B|)$ time.
\end{lemma}
\begin{proof}
We first recall the multiple-source shortest path algorithm
of Klein~\cite{klein:mssp}.
Given a brick $B$ with $V(\prm B) = \{v_1,v_2,\ldots,v_s\}$
and vertices $v_i$ appearing on $\prm B$ clockwise in this order, the algorithm computes in
$\Oh(|B| \log |B|)$ time a shortest-path tree $T(v_i)$
for each vertex $v_i$.
However, as the total size of all these shortest-path trees is $\Omega(|B|^2)$,
they are computed implicitly.
More precisely, in~\cite{klein:mssp} it is shown that in the sequence of rooted trees
$T(v_1),T(v_2),\ldots,T(v_s)$ each edge of $B$ is added to a tree or removed from a tree
only a constant number of times, and the algorithm of~\cite{klein:mssp} computes
in the promised time the sequence of these changes.

\newcommand{\Hcons}{H^{\star}}

We will compute the graph $H$ using an auxiliary variable graph $\Hcons$, initially setting $\Hcons:=\prm B$. At the end of the algorithm, we will have $H=\Hcons$.
The algorithm traverses the path $\north$ from $\Bleft$ to $\Bright$, running the algorithm of~\cite{klein:mssp} to maintain a shortest-path tree $T(v)$ from the currently considered vertex $v\in V(\north)$, and computing the union of all the paths $P_{i,j}$ along the way. We will maintain the invariant that once vertex $x_i$ is processed, the graph $\Hcons$ contains $\prm B$ and all the paths $P_{i',j}$ for all $i'\leq i$.

When visiting a vertex $v \in V(\north)$, apart from the tree $T(v)$
maintained by the algorithm of~\cite{klein:mssp},
we also maintain the graph $T(v) \cap E(\Hcons)$. This graph is a forest, so we may maintain it as a dynamic forest in a standard manner,
e.g., using ET-trees~\cite{ETtrees}, which allows edge addition and removal in $\Oh(\log |B|)$
time. Moreover, each tree of $T(v) \cap E(\Hcons)$ keeps track of its closest to root vertex in $T(v)$;
observe that this information is easy to update upon one edge modification in $T(v)$,
since such a modification always affects at most two trees in the forest $T(v) \cap E(H)$.

Assume now that we consider $v = x_i$ for some $0 \leq i \leq q$. Having updated $T(x_i)$ and $T(x_i)\cap E(\Hcons)$, we would like to add to $\Hcons$ all the edges of $\bigcup_{-r_\leftarrow(i) \leq j \leq r_\rightarrow(i)}E(P_{i,j})$ that are not yet present in $\Hcons$. We first compute all the vertices $z_{i,j}$ for $-r_\leftarrow(i) \leq j \leq r_\rightarrow(i)$: each $z_{i,j}$ can be found in $\Oh(\log |B|)$ time using binary search, provided that for each vertex of $\south$ we precomputed its distance from $\Bleft$ on $\south$. Now, for each $j$, $-r_\leftarrow(i) \leq j \leq r_\rightarrow(i)$, we define the cord $P_{i,j}$ as the path between $z_{i,j}$ and $x_i$ in the tree $T(x_i)$.

The procedure of adding the edges of $\bigcup_{-r_\leftarrow(i) \leq j \leq r_\rightarrow(i)}E(P_{i,j})$ that are not yet present in $\Hcons$ will use $\Oh(\log |B|)$ time per each added edge, and thus the total time spent on running all these procedures will be $\Oh(|B|\log |B|)$. The update of $\Hcons$ is done as follows. For each $j$, we traverse the tree $T(x_i)$ from $z_{i,j}$ up to the root $x_i$, adding to $\Hcons$ the edges that are missing in $\Hcons$, and update $T(x_i)\cap E(\Hcons)$ upon each such addition. When traversing the tree, however, we do not consider edges that are already present in $\Hcons$: using the fact that every component $C$ of $T(x_i) \cap E(H)$ remembers its closest to the root vertex in $T(x_i)$, we may always jump immediately to this vertex, and thus process only edges that are not yet in $\Hcons$.

Thus, the total work of the algorithm consists of summand $\Oh(|B|\log |B|)$ for running the algorithm of~\cite{klein:mssp}, summand $\Oh(|B|\log |B|)$ for maintaining the dynamic forest $T(v) \cap E(\Hcons)$ upon modifications of $T(v)$ and of $E(\Hcons)$, and summand $\Oh(\eps^{-2}|B|\log |B|)$ for computing all the vertices $z_{i,j}$ for all $1\leq i\leq q$ and $-r_\leftarrow(i) \leq j \leq r_\rightarrow(i)$. The running time follows.
\end{proof}

By appropriately rescaling the accuracy parameter $\eps$,
we complete the proof of Theorem~\ref{thm:wei:strips}, and thus of Theorem~\ref{thm:wei:paths}.


